CryoHype: Reconstructing a thousand cryo-EM structures with transformer-based hypernetworks

Cryo-electron microscopy (cryo-EM) is an indispensable technique for determining the 3D structures of dynamic biomolecular complexes. While typically applied to image a single molecular species, cryo-EM has the potential for structure determination of many targets simultaneously in a high-throughput fashion. However, existing methods typically focus on modeling conformational heterogeneity within a single or a few structures and are not designed to resolve compositional heterogeneity arising from mixtures of many distinct molecular species. To address this challenge, we propose CryoHype, a transformer-based hypernetwork for cryo-EM reconstruction that dynamically adjusts the weights of an implicit neural representation. Using CryoHype, we achieve state-of-the-art results on a challenging benchmark dataset containing 100 structures. We further demonstrate that CryoHype scales to the reconstruction of 1,000 distinct structures from unlabeled cryo-EM images in the fixed-pose setting.

==> Tables/fsc_noiseless.tex <==
% \begin{table}
%   \centering
%   \footnotesize
%   \caption{\textbf{AUC of Per-Image FSC (Noiseless).} The metrics are computed after masking out background noise. Standard deviation of all AUC-FSCs per method is given in parentheses. Metrics for backprojection are provided to give an upper bound on reconstruction quality.}
%   \vspace{-7pt}
%   \resizebox{0.9\textwidth}{!}{
%       \begin{tabular}{c|c|c|c|c}
%         \toprule
        
%         \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{|c|}{\textbf{IgG-RL}} & \multicolumn{2}{|c}{\textbf{Tomotwin-100}} \\
%         \cmidrule(r){2-5}
%         % \cmidrule(r){2-5} \cmidrule(l){7-10}
%         & Mean (std) & Median & Mean (std) & Med \\
%         \midrule
%         CryoDRGN \cite{zhong2021cryodrgn} & 0.353 (0.015) & 0.353 & 0.328 (0.022) & 0.327\\
%         % \midrule
%         % Ours (single-view) & 0.413 (0.007) & 0.411 & 0.384 (0.019) & 0.387 & 0.385 (0.03) & 0.384 \\
%         \textbf{CryoHype} & \textbf{0.414 (0.007)} & \textbf{0.412} & \textbf{0.393 (0.018)} & \textbf{0.395}\\
%         \midrule
%         Backprojection & 0.418 (0.007) & 0.416 & 0.406 (0.018) & 0.406 \\
%         \bottomrule
%       \end{tabular}
%     }
%     \label{tab:tab_per-img_nonoise}
%     \vspace{-5pt}
% \end{table}

% CryoDRGN (Noiseless)),SUMMARY,6.0,mean=1.9750; med=1.9165; std=0.4450,mean=0.6513; med=0.6534; std=0.0540
% CryoHype (Noiseless),SUMMARY,6.0,mean=1.8663; med=1.9002; std=0.2514,mean=0.6564; med=0.6512; std=0.0375
% CryoDRGN (Noiseless)),SUMMARY,5.0,mean=1.6120; med=1.5854; std=0.3233,mean=0.7042; med=0.7045; std=0.0457
% CryoHype (Noiseless),SUMMARY,5.0,mean=1.6571; med=1.6975; std=0.2537,mean=0.6985; med=0.6925; std=0.0374
% Backprojection,SUMMARY,5.0,mean=1.2499; med=1.2653; std=0.1977,mean=0.7339; med=0.7311; std=0.0419

% \begin{table}
%   \centering
%   \footnotesize
%   \caption{\textbf{AUC of Per-Image FSC (Noiseless).} The metrics are computed after masking out background noise. Standard deviation of all AUC-FSCs per method is given in parentheses. Metrics for backprojection are provided to give an upper bound on reconstruction quality.}
%   \vspace{-7pt}
%   \resizebox{0.9\textwidth}{!}{
%       \begin{tabular}{c|c c|c c|c c|}
%         \toprule
        
%         \multirow{2}{*}{\textbf{Method}} & \multicolumn{6}{|c|}{\textbf{Tomotwin-100}} \\
%         \cmidrule(r){2-7}
%         % \cmidrule(r){2-5} \cmidrule(l){7-10}
%         & Mean (std) & Med & $\downarrow$ CD (std) & Med & $\uparrow$ vIoU (std) & Med \\
%         \midrule
%         CryoDRGN \cite{zhong2021cryodrgn} & 0.328 (0.022) & 0.327 & \textbf{1.6120 (0.3233)} & \textbf{1.5854} & \textbf{0.7042 (0.0457)} & \textbf{0.7045}\\
%         % CryoDRGN \cite{zhong2021cryodrgn} & 0.328 (0.022) & 0.327 & 1.9750 (0.4450) & 1.9165 & 0.6513 (0.0540) & \textbf{0.6534}\\
%         % \midrule
%         % Ours (single-view) & 0.413 (0.007) & 0.411 & 0.384 (0.019) & 0.387 & 0.385 (0.03) & 0.384 \\
%         \textbf{CryoHype} & \textbf{0.384 (0.019)} & \textbf{0.387} & 1.6571 (0.2537) & 1.6975 & 0.6985 (0.0374) & 0.6925 \\
%         % \textbf{CryoHype} & \textbf{0.384 (0.019)} & \textbf{0.387} & \textbf{1.8663 (0.2514)} & \textbf{1.9002} & \textbf{0.6564 (0.0375)} & 0.6512 \\
%         % \midrule
%         Backprojection & 0.406 (0.018) & 0.406 & 1.2499 (0.1977) & 1.2653 & 0.7339 (0.0419) & 0.7311 \\
%         \bottomrule
%       \end{tabular}
%     }
%     \label{tab:tab_per-img_nonoise}
%     \vspace{-5pt}
% \end{table}

\begin{table*}
  \centering
  \footnotesize
  \caption{\textbf{Quantitative performance on Tomotwin-100 (Noiseless)}, measured by $\mathrm{FSC}_{\mathrm{AUC}}$, CD, and vIoU. Metrics are also computed on backprojected images for each G.T. structure as an upper bound.}
  % \vspace{-7pt}
  \resizebox{0.9\textwidth}{!}{
      \begin{tabular}{c|c c|c c|c c}
        \toprule
        
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{6}{|c}{\textbf{Noiseless Tomotwin-100}} \\
        \cmidrule(r){2-7}
        % \cmidrule(r){2-5} \cmidrule(l){7-10}
        & $\uparrow$ Mean $\mathrm{FSC}_{\mathrm{AUC}}$ (std) & Median & $\downarrow$ Mean CD (std) & Med & $\uparrow$ Mean vIoU (std) & Med \\
        \midrule
        % CryoDRGN \cite{zhong2021cryodrgn} & 0.328 (0.022) & 0.327 & \textbf{1.6120 (0.3233)} & \textbf{1.5854} & \textbf{0.7042 (0.0457)} & \textbf{0.7045}\\
        CryoDRGN \cite{zhong2021cryodrgn} & 0.328 (0.022) & 0.327 & 1.9750 (0.4450) & 1.9165 & 0.6513 (0.0540) & \textbf{0.6534}\\
        % \midrule
        % Ours (single-view) & 0.413 (0.007) & 0.411 & 0.384 (0.019) & 0.387 & 0.385 (0.03) & 0.384 \\
        % \textbf{CryoHype} & \textbf{0.384 (0.019)} & \textbf{0.387} & 1.6571 (0.2537) & 1.6975 & 0.6985 (0.0374) & 0.6925 \\
        \textbf{CryoHype} & \textbf{0.384 (0.019)} & \textbf{0.387} & \textbf{1.8663 (0.2514)} & \textbf{1.9002} & \textbf{0.6564 (0.0375)} & 0.6512 \\
        \midrule
        Backprojection & 0.406 (0.018) & 0.406 & 1.1931 (0.1987) & 1.2130 & 0.7527 (0.0406) & 0.7500 \\
        \bottomrule
      \end{tabular}
    }
    \label{tab:tab_per-img_nonoise}
    % \vspace{-10pt}
\end{table*}

==> Tables/new_metrics.tex <==
% \begin{table*}[t]
%   \centering
%   \footnotesize
%   \caption{\textbf{3D Reconstruction Metrics (Noisy).} Metrics are computed after background masking, with standard deviations per method in parentheses. Chamfer distance is given in angstroms (\r{A}). Isosurface levels are set at 1.5 for IgG-RL and 5.0 for Tomotwin-100. \TODO{update with single-view results}}
%   \resizebox{0.9\textwidth}{!}{
%       \begin{tabular}{c|c c|c c|c c|c c}
%         \toprule   
%         \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{|c|}{\textbf{IgG-RL}} & \multicolumn{4}{|c}{\textbf{Tomotwin-100}} \\
%         \cmidrule(r){2-9}
%         & $\downarrow$ CD (std) & Median & $\uparrow$ vIoU (std) & Med & $\downarrow$ CD (std) & Med & $\uparrow$ vIoU (std) & Med \\
%         \midrule
%         CryoDRGN \cite{zhong2021cryodrgn} & 5.158 (3.900) & 3.768 & 0.578 (0.069) & 0.518 & 1.798 (1.142) & \textbf{1.608} & 0.690 (0.070) & \textbf{0.703} \\
%         CryoHype & \textbf{1.566 (0.082)} & \textbf{1.569} & \textbf{0.708 (0.015)} & \textbf{0.706} & \textbf{1.645 (0.270)} & 1.683 & \textbf{0.702 (0.037)} & 0.698 \\
%         \bottomrule
%       \end{tabular}
%     }
%     \label{tab:tab_recon_metrics}
% % \vspace{-14pt}
% \end{table*}

\begin{table*}[t]
  \centering
  \footnotesize
  \caption{\textbf{3D Reconstruction Metrics (Noisy).} Metrics are computed after background masking, with standard deviations per method in parentheses. Chamfer distance is given in angstroms (\r{A}). Isosurface levels are set at 1.5 for IgG-RL and 5.0 for Tomotwin-100. \TODO{update with single-view results}}
  \resizebox{0.9\textwidth}{!}{
      \begin{tabular}{c|c c|c c}
        \toprule   
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{|c}{\textbf{Tomotwin-100}} \\
        \cmidrule(r){2-5}
        &  $\downarrow$ CD (std) & Med & $\uparrow$ vIoU (std) & Med \\
        \midrule
        CryoDRGN \cite{zhong2021cryodrgn} & 1.798 (1.142) & \textbf{1.608} & 0.690 (0.070) & \textbf{0.703} \\
        CryoHype & \textbf{1.645 (0.270)} & 1.683 & \textbf{0.702 (0.037)} & 0.698 \\
        \bottomrule
      \end{tabular}
    }
    \label{tab:tab_recon_metrics}
% \vspace{-14pt}
\end{table*}

==> Tables/shapenet_em.tex <==
\begin{table}
  \centering
  \footnotesize
  \caption{\textbf{AUC of Per-Image FSC (Noisy).} The metrics are computed after masking out background noise. Standard deviation of all AUC-FSCs per method is given in parentheses. The best result in each section is \textbf{bolded} and the second-best result is \underline{underlined}. $\dagger$ indicates that the result is from \cite{jeon2024cryobench}.}
  \vspace{-5pt}
  \resizebox{0.48\textwidth}{!}{
      \begin{tabular}{c|c|c|c|c}
        \toprule
        
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{|c|}{\textbf{IgG-RL}} & \multicolumn{2}{|c}{\textbf{Tomotwin-100}}  \\
        \cmidrule(r){2-5}
        % \cmidrule(r){2-5} \cmidrule(l){7-10}
        & Mean (std) & Median & Mean (std) & Med \\
        \midrule
        CryoDRGN \cite{zhong2021cryodrgn} & 0.331 (0.016)$^\dagger$ & 0.333$^\dagger$ & 0.316 (0.046)$^\dagger$ & 0.321$^\dagger$  \\
        % CryoDRGN (200 epochs) \cite{zhong2021cryodrgn} & 0.298 (0.022) & 0.303 & 0.346 (0.03) & 0.348 & &  \\
        DRGN-AI-fixed \cite{levy2024revealing} & 0.348 (0.012)$^\dagger$ & 0.350$^\dagger$ & 0.202 (0.044)$^\dagger$ & 0.207$^\dagger$\\
        Opus-DSD \cite{luo2023opus} & 0.343 (0.016)$^\dagger$ & 0.346$^\dagger$ & 0.237 (0.049)$^\dagger$ & 0.251$^\dagger$\\
        % \textbf{Ours (single-view)} & 0.346 (0.006) & 0.345 & \underline{0.346 (0.033)} & \underline{0.353} &  & \\
        3DFlex~\cite{punjani20233dflex} & 0.337 (0.007)$^\dagger$ & 0.337$^\dagger$ & - & -\\
        3DVA \cite{punjani20213d} & 0.333 (0.014)$^\dagger$ & 0.335$^\dagger$ & 0.088 (0.040)$^\dagger$ & 0.077$^\dagger$\\
        RECOVAR \cite{gilles2023bayesian} &\textbf{0.363} (0.011)$^\dagger$ & \textbf{0.363}$^\dagger$ & 0.258 (0.109)$^\dagger$ & 0.254$^\dagger$\\
        3D Class. \cite{punjani2017cryosparc} & 0.309 (0.01)$^\dagger$ & 0.307$^\dagger$ & 0.046 (0.026)$^\dagger$ & 0.037$^\dagger$ \\
        \midrule
        \textbf{CryoHype} & \textbf{0.363 (0.005)} & \underline{0.362} & \textbf{0.377 (0.018)} & \textbf{0.377} \\
        \midrule
        Backprojection & 0.334 (0.004) & 0.333 & \underline{0.364 (0.023)} & \underline{0.364}  \\
        \bottomrule
      \end{tabular}
    }
    \vspace{-15pt}
    \label{tab:tab_per-img_snr001}
% \vspace{-14pt}
\end{table}

==> TexFigures/ambris_dataset.tex <==
\begin{figure*}[tb]
  \centering
  \includegraphics[width=0.9\linewidth]{Figures/Tomotwin-500.pdf}
  \caption{\textbf{\dataset/.} Example atomic models, density maps, and projected images from \texttt{\dataset/}, containing 1000 distinct structures. }
  %First, 1000 atomic models are curated from Cryo2Struct~\citep{giri2024cryo2structdata} by molecular weight. We then create density maps by simulating the cryo-EM formation model (Eqn.~\ref{eqn:real-img-form}) and project to create simulated images. We do not use Cryo2Struct's density maps because they are extremely inconsistent. }
  \label{fig:ambris-dataset}
  \vspace{-15pt}
\end{figure*}

==> TexFigures/motivation.tex <==
\begin{figure*}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Figures/rebuttal/combined_vis_acts3.png}
  \caption{UMAP of activations from the penultimate layer of the neural field decoder}
  \label{fig:activations}
\end{subfigure}%
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=.4\textwidth]{Figures/rebuttal/fc0_log10_v3.png}
  \caption{Log-standard deviations of first-layer weights}
  \label{fig:first-layer}
\end{subfigure}
\caption{In (a), \method/ has greater diversity in their intermediate activations comapred to CryoDRGN, and (b) \method/'s neural field has much greater variation in first layer weights compared to CryoDRGN's neural field.}
\label{fig:motivation}
\end{figure*}

==> TexFigures/new_metrics.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.9\linewidth]{Figures/3d_reconstruction_metrics.pdf}
  \caption{\textbf{3D Reconstruction Metrics across Isosurface Levels.} Each curve shows the average CD ($\downarrow$) or vIoU ($\uparrow$) across all conformations with error bars indicating the standard deviation. Colors correspond to methods shown in the legend.}
  % Table \ref{tab:tab_recon_metrics} presents the corresponding metrics at an isosurface level of 1.5 for IgG-RL and 5.0 for Tomotwin-100, respectively.}
  \label{fig:3d_recon_metrics}
  \vspace{-20pt}
\end{figure}

==> TexFigures/new_metrics_shapenet.tex <==
\begin{figure}
  \centering
  \includegraphics[width=1.0\linewidth]{Figures/3d_reconstruction_metrics.pdf}
  \caption{\textbf{Quantiative results on the ShapeNet-EM dataset.} CryoHype does a better job of capturing the correct structural details than CryoDRGN.}
  \label{fig:shapenet}
\end{figure}

==> TexFigures/nv_generalization.tex <==
\begin{figure}
  \centering
  \includegraphics[width=1.0\linewidth]{Figures/3d_reconstruction_metrics.pdf}
  \caption{\textbf{Unseen views.} CryoHype generalizes far better to unseen views than CryoDRGN, which fails to produce reasonable reconstructions.}
  \label{fig:unseen_view}
  \vspace{-20pt}
\end{figure}

==> TexFigures/overview.tex <==
\begin{figure*}[htb!]
  \centering
  \includegraphics[width=0.99\linewidth]{Figures/cryohype_pullfigure.pdf}
  \caption{\textbf{Overview of our approach.} (a) Goal of cryo-EM reconstruction. Previously, research has primarily focused on addressing conformational heterogeneity, which arises from shape deformations within a \textit{single} protein. In contrast, our approach aims to tackle more complex forms of heterogeneity, which stems from variations in the composition of \textit{diverse} protein complexes, using new methods and larger-scale datasets. (b) Overview of our approach. The components in green show show our contributions over past deep learning methods. 
  % (c) Analysis with various metrics are provided, including Chamfer Distance (CD), Intersection-over-Union (IoU), per-image FSC, and latent space visualization (Latent).
  }
  % \vspace{-10pt}
  \label{fig:pull-figure}
\end{figure*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

